Pre-analysis protocol for an observational study on the effects of adolescent sports participation on health in early adulthood

We will study the impact of adolescent sports participation on early-adulthood health using longitudinal data from the National Study of Youth and Religion. We focus on two primary outcomes measured at ages 23--28 -- self-rated health and total score on the PHQ9 Patient Depression Questionnaire -- and control for several potential confounders related to demographics and family socioeconomic status. Comparing outcomes between sports participants and matched non-sports participants with similar confounders is straightforward. Unfortunately, an analysis based on such a broad exposure cannot probe the possibility that participation in certain types of sports (e.g., collision sports like football or soccer) may have larger effects on health than others. In this study, we introduce a hierarchy of exposure definitions, ranging from broad (participation in any after-school organized activity) to narrow (e.g., participation in limited-contact sports). We will perform separate matched observational studies, one for each definition, to estimate the health effects of several levels of sports participation. In order to conduct these studies while maintaining a fixed family-wise error rate, we deployed an ordered testing approach that exploits the logical relationships between exposure definitions. Our study will also consider several secondary outcomes including body mass index, life satisfaction, and problematic drinking behavior.

==> abstract.tex <==
\begin{abstract}
We will study the impact of adolescent sports participation on early-adulthood health using longitudinal data from the National Survey of Youth and Religion.
We focus on two primary outcomes measured at ages 23--28 --- self-rated health and total score on the PHQ9 Patient Depression Questionnaire --- and control for several potential confounders related to demographics and family socioeconomic status.
Comparing outcomes between sports participants and matched non-sports participants with similar confounders is straightforward.
Unfortunately, an analysis based on such a broad exposure cannot probe the possibility that participation in certain types of sports (e.g. collision sports like football or soccer) may have larger effects on health than others. 

In this study, we introduce a hierarchy of exposure definitions, ranging from broad (participation in any after-school organized activity) to narrow (e.g. participation in limited-contact sports).
We will perform separate matched observational studies, one for each definition, to estimate the health effects of several levels of sports participation.
In order to conduct these studies while maintaining a fixed family-wise error rate, we developed an ordered testing approach that exploits the logical relationships between exposure definitions.
Our study will also consider several secondary outcomes including body mass index, life satisfaction, and problematic drinking behavior. 
\end{abstract}
